PlaMo: Plan and Move in Rich 3D Physical Environments

Controlling humanoids in complex physically simulated worlds is a long-standing challenge with numerous applications in gaming, simulation, and visual content creation. In our setup, given a rich and complex 3D scene, the user provides a list of instructions composed of target locations and locomotion types. To solve this task we present PlaMo, a scene-aware path planner and a robust physics-based controller. The path planner produces a sequence of motion paths, considering the various limitations the scene imposes on the motion, such as location, height, and speed. Complementing the planner, our control policy generates rich and realistic physical motion adhering to the plan. We demonstrate how the combination of both modules enables traversing complex landscapes in diverse forms while responding to real-time changes in the environment. Video: https://youtu.be/wWlqSQlRZ9M .

==> SIGGRAPH_2024/background.tex <==
\section{Preliminaries}
We begin with a formal introduction of the reinforcement learning (RL) setup for training our motion controller, together with the mathematical representation of our simulated scene. 
\subsection{Reinforcement Learning}
In this work, we train a sparsely-constrained motion controller. We model this as a RL \cite{sutton2018reinforcement} problem, where an agent interacts with an environment according to a policy $\pi$. At each step $t$, the agent observes a state $s_t$ and samples an action $a_t$ from the policy $a_t \sim \pi (a_t | s_t)$. The environment then transitions to the next state $s_{t+1}$ based on the transition probability $p(s_{t+1} | s_t, a_t)$. The goal is to maximize the discounted cumulative reward, defined as
\begin{equation*}
    J = \mathbb{E}_{p(\sigma|\pi)} \left[ \sum_{t=0}^T \gamma^t r_t \middle| s_0 = s \right] \,,
\end{equation*}
where $p(\sigma|\pi) = p(s_0) \Pi_{t=0}^{T-1} p(s_{t+1}|s_t,a_t) \pi(a_t | s_t)$ is the likelihood of a trajectory $\sigma = (s_0, a_0, r_0, \ldots, s_{T-1}, a_{T-1}, r_{T-1}, s_T)$, and $\gamma \in [0, 1)$ is a discount factor that determines the effective horizon of the policy.

To find the optimal policy $\pi^*$ that maximizes the discounted cumulative reward, the popular policy gradient paradigm seeks to directly optimize the policy using the utility of complete trajectories. Perhaps the most widely used algorithm in this context is PPO \cite{schulman2017proximal}, which gradually improves the policy while maintaining stability without drifting too far from it.

In this work, the state of the system consists of the humanoid's pose and speed, in addition to the scene information, such as the surrounding height map. As we focus on physics-based animation, the actions correspond to motor actuations for the simulated humanoid.



\begin{figure*}[ht]
    \centering
    \includegraphics[width=\linewidth]{figures/method_overview.png}
    \caption{\textbf{Method overview.}  %\gal{Lets use input green boxes consistently. sampels should be both outside (or inside)} 
     A simulated scene is provided to the path planner, together with a series of textual instructions, requesting a humanoid to reach landmarks in the scene using various locomotion types. The high-level planner computes a path that is fed to a reinforcement-learning-based low-level motion controller, which controls a humanoid to follow the path using the request locomotion type.}
    \label{fig:overview}
\end{figure*}


\subsection{Humanoid control for animation}
We consider physically animated humanoids interacting within a simulated world. Here, the rules of physics, such as gravity and collisions, ensure the realism of the generated animation. The humanoids are defined by the location and orientation of their joints (head, torso, arms etc.) and they are controlled using PD controllers located in each of the joints. The humanoid dynamics follow rigidity and anatomical constraints. 

We describe the simulated scene our agent lives in as follows:
\begin{equation}\label{eq:scene}
\textit{Scene}=\{h, \mathcal{O}_\text{static}, \mathcal{O}_\text{dynamic}, \mathcal{O}_\text{top},  \mathcal{L}\}
\end{equation}
\begin{enumerate}
    \item A terrain given as a height map $h(x,y) \in \mathbb{R}$, specifying the height for each location in the grid. 
    \item A set of non-passable static obstacles  $\mathcal{O}_\text{static}$.
    \item A set of dynamic obstacles and their dynamics $\mathcal{O}_\text{dynamic}$.
    \item A set of height-limiting (``top'') obstacles requiring the agent to crouch or crawl when traversing through them $\mathcal{O}_\text{top}$. 
    \item A set of landmarks $\mathcal{L}=\{L_i\}_{i=0}^l.$    
\end{enumerate}
Each time-step of the simulation corresponds to the positions and speeds of all objects in the scene, and a rendered frame of the scene. An actuation is given by the controller on the humanoid, the location of dynamic obstacles are updated by a pre-specified rule, and the simulation advances according to physics to the next time-step.

% When learning to control a humanoid to perform tasks for animation purposes, it is critical to provide it with additional guidance so the resulting movements look natural. This is commonly done using a discriminator trained on real world motion captures, in this sense we closely follow AMP \cite{peng2021amp} and denote its discriminator reward by $r^\text{amp}$. 
In our work, the requested task is a short-horizon XYZ path with a fixed time interval between each two subsequent waypoints in the path:
\begin{equation*}
    \tau =\left( x^t, y^t, z^t \right)_{t=0}^T,
\end{equation*}
for a fixed horizon $T \in \mathbb{N}$.

Finally, the higher-level goal is to travel a desired path between a series of landmarks $L_1, \dots, L_k$ according to their order.


==> SIGGRAPH_2024/discussion.tex <==
\section{Discussion, limitations and future work}\label{sec: limitations}
In this paper, we described \ourmethod{}, a framework for path and motion planning of humanoids in simulated environments for physics-based animation. Given a complex simulated scene with landmarks, combined with requested locomotion, the planner generates a path to successfully navigate through a sequence of target landmarks. This takes into account not only the scene information, such as walls, 3D obstacles and dynamic obstacles, but also the character's performance envelope. We show that our controller successfully tracks these paths, producing complex and realistic  motions. 

\ourmethod{} allows flexibility in the scenes it can handle, but it has various limitations which we outline below as future work. 

\textbf{Interaction with objects and multiple agents. } We focused on controlling the motion of a single agent. Many interesting scenarios for gaming and simulation would require physical interactions with dynamic objects or other agents. Learning such interactions not only requires specific data, but may require extending the human model and potentially the controller training, for example with hands \cite{SMPL-X:2019}. 

\textbf{Dynamic objects. } We handled dynamic objects with simple motion that can be easily predicted using rules. odelling more complex dynamic objects may require learning-based approaches to model the dynamic scene. %When dynamic obstacles move in a known or at least predictable manner, planning around them can be done with rule-based approaches. However, this is not the case in scenes with unpredictable obstacles. For example other players, or even when given objects that simulating their future path is costly (such as a rock rolling down rich terrain). To cope with this challenge, as our planner is composed of several modules, part of them can be replaced with learned components. %Such can be handled by learnable dynamic planner, for example a diffusion model for path generation.

%\textbf{More diverse motion styles.} In this work we devise a framework for solving three-dimensional locomotion problems. However, often high-level control may not be enough, and the user may want to control intricate details of the style for example: ``walk happily", ``dance" or ``run like a zombie".

%Extending the physical model to include additional modes of movement while maintaining reasonable locomotion capabilities is hard and requires additional research.

\textbf{Rich language and scene understanding. } The focus of the current paper was on planning and control, given templated language instructions and full knowledge about the visual scene. It allows us to showcase the system in complex, yet pre-defined scenes. Large language models and visual models can provide a means for combining research on scene understanding with \ourmethod{}, to generate complex locomotion in previously unseen scenes with zero user interaction. % Integration of a large language model into the system will provide strong capabilities in parsing free text for route guidance or incorporating the motion labels into the training process.

With these expansions in mind, we see \ourmethod{} as a stepping stone in a much greater system where non-playable characters (NPCs) are given roles to play, forming a rich simulated virtual world.


% No objects yet. Can't control intricate details of the motion, just high-level stuff.
% Path planner isn't learned. While this matches what many games utilize, it doesn't anticipate what will happen in a dynamic game with less predictable objects which we don't control (such as other players).
% Semantic planner isn't a strong integration of an LLM into the loop.

%\section{Discussion and future work}
%Although physics-based animation is harder than kinematic animation, as research progresses the gap between the two closes, enabling physical models to animate increasingly more complex tasks in diverse environments. To do so, more complex decision making frameworks will be required beyond simple motion control such as navigation, obstacle avoidance and speed tuning. 

% Physics-based animation has demonstrated impressive results in motion diversity, object interaction, handling of uneven terrains and user control. Still, performing complex tasks in diverse environments requires higher level decision for navigation, obstacle avoidance and speed tuning. One framework which envelopes all levels of control is required to make physical animation a helpful and powerful tool in the applications of this technology. In this work we wrap the motion controller within such a framework, demonstrating a humanoid character that can perform a list of instructions in a rich physics-based simulation environment. This may be another stepping stone in a much greater system where non-playable characters (NPCs) are given roles to play, forming a rich simulated virtual world.

% Our framework is modular, allowing improvements in the high-level planning or the low level movement model without changing its flow. Thus, textual guidance can be replaced with a more elaborate free text language model, the motion controller can be improved to support movement styles, and dynamic obstacle avoidance can be done with a diffusion model. Other exciting extensions are interactions with objects and other agents, and text based scene generation.


%In this work, we presented \ourmethod{}, a system comprising of a motion planner and a locomotion controller. Provided a complex scene and a sequence of waypoints, combined with requested locomotion, the planner generates a path to successfully reach the target landmark. This takes into account not only the scene information, such as walls and top obstacles, in addition to dynamic obstacles, but also the character's performance envelope. We show that our controller successfully tracks these paths, and as a result, produces complex and rich motions. We see PlaMo as a stepping stone in a much greater system where non-playable characters (NPCs) are given roles to play, forming a rich simulated virtual world.

% Our framework is modular, allowing plug-and-play improvements in the high-level planning and the low-level movement model. This, for example, may enable the integration of an elaborate free-text language model. In addition, the motion controller can be improved to support movement styles, and dynamic obstacle avoidance can be done with a diffusion model. Other exciting extensions are interactions with objects and other agents, and text-based scene generation.


\newpage

==> SIGGRAPH_2024/experiments.tex <==

\section{Experiments}\label{sec: experiments}

% Explain what we will show in the experiments

% Complementing the numerical evaluations, we provide video demonstrations and comparisons in the supplementary material.

% Explain about the data

% Explain about the humanoid model. Can copy from CALM/PADL/ASE.
We test \ourmethod{} both qualitatively and quantitatively. 
First, we evaluate the motion controller with several common forms of motion across a range of randomized terrains. In addition, we evaluate our design decision regarding the workflow for training the controller, using ablation experiments regarding both data curation and height-speed coupled path generation.

Then, we analyze the quality of the path planner. We focus on evaluating the paths produced by the QP solver in terms of how well they fit the capability envelope of the locomotion controller.
Finally, we provide qualitative examples both for the locomotion controller and the whole system in a complex scene with multiple landmarks. We stress that our test scenes were not observed during training. Our agent can navigate during inference in every scene as defined in \eqref{eq:scene}, without requiring any further training.
% We show that our methods outperform baselines, and result in a smooth and visually pleasing humanoid motion in diverse scenes. 
Video demonstrations and comparisons are provided in the supplementary material. 

\subsection{Experiment details}

\textbf{Simulation.} To simulate our physical environment, we used IsaacSim\footnote{NVIDIA Isaac Sim. Available online: \hyperlink{https://developer.nvidia.com/isaac-sim}{https://developer.nvidia.com/isaac-sim}}. The controllers make decisions at a rate of $30 \left[Hz\right]$, while the simulation runs at $60 \left[Hz\right].$ We train the motion controller for 7 days on a single NVIDIA V100 GPU. 

\textbf{Training Data. } To train our motion controller to perform realistic motions, we utilize motion capture data from the AMASS dataset \cite{AMASS:ICCV:2019} that contains more than 10 hours of diverse motion capture data, consisting of thousands of distinct motions. Complementing AMASS, \citet{guo2022generating} provide 3 textual labels for each motion. 

\textbf{Training procedure.} All training data from AMASS were recorded on a flat terrain. To train on uneven terrain, we sample different types of terrains: slopes, stairs and gravel. We then let the agent follow random paths on each. The motions we curated contained only locomotion on flat ground, without object interaction (stepping on boxes) or other (such as going up stairs).%As was seen in AMP \cite{peng2021amp}, the discriminator can easily adapt the motion to look realistic on uneven terrains. 


\subsection{Data purification strategies}

Although training on the entire AMASS dataset is possible, many motions in that dataset are irrelevant to locomotion, such as performing hand gestures or dancing. Since the reward in our model is discriminative in nature \cite{peng2021amp}, training with a data distribution that does not match the task distribution may result in uncanny or even bad motions. In this work, we tested two methods of data purification, which we compare here in an ablation study. 

First, we use a large language model (LLM, ChatGPT4 \cite{openai2023gpt}). We provide it with the textual descriptions of each movement and ask it to categorize the motions into five classes: [`walking', `running', `crouching', `crawling', others]. This filtering reduced the size of dataset down to 600 motions. We then also tested a manual curation procedure. Here, we handpick 75 motion captures, roughly 20 from each desired motion type, and create a small, tailor-made dataset. In our studies, we also compare our motion-aware path sampler that samples the requested speed along a random path according to the requested height, with a simple baseline of uncoupled sampling of both speed and height. 


\begin{table}[hb]
    \centering
    \caption{\textbf{Locomotion ablation.} We compare various design choices for both data purification and path generation during training. The analysis focuses on crawling on rough terrain, with additional results provided in the supplementary material. The results were averaged over $10^6$ runs.}
    \begin{tabular}{l|c||c|c}
                    % & \multicolumn{2}{c}{\textbf{Crawl}}  \\ \toprule 
                   Data purification & Path generator & XY-err & Z-err \\ \toprule
         \multicolumn{2}{c|}{\textbf{Ours} (Curated + Coupled)} & 0.25 & 0.10 \\ \hline
         Curated & Naive path generator &  0.50 & 0.13 \\ \hline
         Naive & Naive  & 0.78 & 0.09 \\ \hline
         Naive & Coupled  & 1.16 & 0.17 \\ \hline
         None & Coupled  & 0.66 & 0.09 \\ \hline
         None & Naive  & 1.39 & 0.19
    \end{tabular}
    \label{tab: locomotion ablation}
\end{table}


\begin{table*}[ht]
    \centering
    \caption{\textbf{Mean path displacement for various locomotion types .} We test four motion types over four types of terrains. For each, we sample a path with constant speed and height, and compute the mean error between the position of the humanoid and the desired path. The results were averaged over $10^6$ runs.}
    \begin{tabular}{l||c|c|c|c|c|c|c|c}
                    & \multicolumn{2}{c|}{\textbf{Crawl }} & \multicolumn{2}{c|}{\textbf{Crouch-walk}} & \multicolumn{2}{c|}{\textbf{Walk}} & \multicolumn{2}{c}{\textbf{Run}}  \\ \toprule 
                   \textbf{Terrain} & XY-err $\left[m\right]$ & Z-err$\left[m\right]$ & XY-err $\left[m\right]$& Z-err $\left[m\right]$& XY-err$\left[m\right]$ & Z-err $\left[m\right]$& XY-err$\left[m\right]$ & Z-err$\left[m\right]$ \\ \hline
        Flat    & 0.20 & 0.07 & 0.20 & 0.03 & 0.24 & 0.21 & 0.52 & 0.26 \\ \hline
        Slope   & 0.21 & 0.09 & 0.22 & 0.03 & 0.25 & 0.21 & 0.60 & 0.27 \\ \hline
        Rough   & 0.25 & 0.10 & 0.25 & 0.04 & 0.29 & 0.24 & 0.79 & 0.31 \\ \hline
        Stairs  & 0.45 & 0.13 & 0.41 & 0.07 & 0.39 & 0.27 & 1.01 & 0.35
    \end{tabular}
    \label{tab: locomotion controller}
\end{table*}


We evaluate the effect of the design decisions of the data purification protocol. In \cref{tab: locomotion ablation}, we focus on the crawl task on rough terrain, because crawling was the hardest type of motion to generate. This is because crawling requires interaction between the humanoid's hands and the terrain, and it is very distinct from most of the AMASS dataset. The results in \cref{tab: locomotion ablation} reveal that the more restrictive the purification of the data, the better the data matches the task distribution, and the better the performance of the test. Specifically, the wesst performance is achieved without any purification (None). Applying  naive purification using an LLM slightly improves, and careful manual curation resulted in the best scores. We also observe that by limiting the requested paths, during training, to those contained in the data (for example, low speeds while crawling), the motion-aware path generator further results in improved performance.

% The controllers make decisions at a rate of 30 Hz, whereas the simulation runs at 60 Hz.

% Additional details, including hyper-parameters, are included in the appendix.

\subsection{Locomotion}\label{exp: locomotion}

We test our locomotion module on various terrains for every motion type; example videos for these are available in the supplementary material, and screen captures are shown in \cref{fig: locomotion example}. In \cref{tab: locomotion controller}, we report the XY-displacement along the path, which shows how well the controller tracks the requested path, and the Z-displacement, which measures how well it maintains the requested height. The results show a hierarchy of complexity between tasks such that stairs are harder than rough gravel-like terrain, which itself is harder than locomotion across a flat and smooth sloped surface. An intriguing result is that, although the data only contained motions traversing flat, smooth floors, the controller learned to generalize to a wide range of uneven terrains and produce robust motions resembling those in the data. Also, as expected, moving at lower speeds enables the character to follow the path more precisely, thus maintaining a lower error. Notice that crouch-walking results in a very small Z error. We attribute this to the phase change between maintaining a very low height while standing and reducing further in height, which requires kneeling. Hence, crouch-walk is a highly constrained motion yielding low variability in the head's height. 



% This is for the appendix
% \begin{table*}[]
%     \centering
%     \begin{tabular}{l|c|c|c|c|c|c|c|c|c}
%                     & & \multicolumn{2}{c|}{\textbf{Crawl}} & \multicolumn{2}{c|}{\textbf{Crouch-walk}} & \multicolumn{2}{c|}{\textbf{Walk}} & \multicolumn{2}{c}{\textbf{Run}}  \\ \toprule 
%                    & Terrain & XY-err & Z-err & XY-err & Z-err & XY-err & Z-err & XY-err & Z-err \\ \hline
%         \multirow{3}{*}{\textbf{Verb74, height first}} & Flat   & 0.20 & 0.07 & 0.20 & 0.03 & 0.24 & 0.21 & 0.52 & 0.26 \\ \cline{2-10}
%          & Rough                                                & 0.25 & 0.10 & 0.25 & 0.04 & 0.29 & 0.24 & 0.79 & 0.31 \\ \cline{2-10}
%          & Stairs                                               & 0.45 & 0.13 & 0.41 & 0.07 & 0.39 & 0.27 & 1.01 & 0.35 \\ \hline\hline
%          \multirow{3}{*}{\textbf{Verb74, naive}} & Flat         & 0.29 & 0.09 & 0.25 & 0.04 & 0.21 & 0.21 & 0.49 & 0.27 \\ \cline{2-10}
%          & Rough                                                & 0.50 & 0.13 & 0.29 & 0.05 & 0.27 & 0.23 & 0.78 & 0.32 \\ \cline{2-10}
%          & Stairs                                               & 0.81 & 0.17 & 0.43 & 0.07 & 0.36 & 0.26 & 0.97 & 0.35 \\ \hline\hline
%          \multirow{3}{*}{\textbf{ChatGPT, height first}} & Flat & 0.67 & 0.06 & 0.25 & 0.06 & 0.25 & 0.23 & 0.57 & 0.29 \\ \cline{2-10}
%          & Rough                                                & 0.78 & 0.09 & 0.32 & 0.07 & 0.34 & 0.26 & 0.85 & 0.35 \\ \cline{2-10}
%          & Stairs                                               & 0.80 & 0.13 & 0.48 & 0.10 & 0.42 & 0.28 & 1.01 & 0.36 \\ \hline\hline
%          \multirow{3}{*}{\textbf{ChatGPT, naive}} & Flat        & 0.62 & 0.15 & 0.26 & 0.05 & 0.29 & 0.27 & 0.60 & 0.30 \\ \cline{2-10}
%          & Rough                                                & 1.16 & 0.17 & 0.37 & 0.07 & 0.35 & 0.28 & 0.87 & 0.36 \\ \cline{2-10}
%          & Stairs                                               & 1.24 & 0.19 & 0.52 & 0.11 & 0.43 & 0.30 & 1.02 & 0.37 \\ \hline\hline
%          \multirow{3}{*}{\textbf{AMASS, height first}} & Flat   & 0.43 & 0.07 & 0.39 & 0.07 & 0.37 & 0.31 & 0.74 & 0.36 \\ \cline{2-10}
%          & Rough                                                & 0.66 & 0.09 & 0.49 & 0.08 & 0.45 & 0.34 & 1.03 & 0.42\\ \cline{2-10}
%          & Stairs                                               & 0.94 & 0.13 & 0.67 & 0.10 & 0.53 & 0.35 & 1.13 & 0.43 \\ \hline\hline
%          \multirow{3}{*}{\textbf{AMASS, naive}} & Flat          & 1.11 & 0.20 & 0.43 & 0.11 & 0.35 & 0.31 & 0.76 & 0.36\\ \cline{2-10}
%          & Rough                                                & 1.39 & 0.19 & 0.53 & 0.13 & 0.44 & 0.34 & 1.06 & 0.40 \\ \cline{2-10}
%          & Stairs                                               & 1.44 & 0.21 & 0.78 & 0.16 & 0.53 & 0.36 & 1.19 & 0.42
%     \end{tabular}
%     \caption{\textbf{Locomotion controller.}}
%     \label{tab: apdx locomotion controller}
% \end{table*}

% First we need to evaluate the most basic model which is the locomotion component.
% Quantitative experiments will show success rate at tracking the path. Need to report average positional error and height error.
% Qualitative experiments need to show how it looks when it's walking/running/crawling. This part is clean without height obstacles or anything dynamic.

\subsection{Speed control}
The third phase of our path planner uses a QP solver to optimize the speed along the path curves. On the one hand, if the speed is too high for the curvature, the character will not be able to maintain the desired route, resulting in large displacement errors and possible collisions with obstacles. On the other hand, if the speed is too low, it will unnecessarily take the character longer to complete the route. The optimization program also considers the maximum acceleration ($a_{\max{}}=0.5 \left[m/s^2\right]$) and deceleration ($a_{\min{}}=-0.1 \left[m/s^2\right]$) physically possible to avoid jerks. 

To demonstrate this trade-off, we designed a ``Slalom'' scene that requires the character to take steep turns. The Slalom scene is depicted in Figure~\ref{fig: slalom}. There, we compare two runs: a constant-speed run versus adaptive speed, as produced by our speed controller module. Both routes are generated using our $A^*$ solver and path refiner. Without adapting the acceleration profile to the curvature of the path, the humanoid fails to follow the path accurately and often collides with the walls. Figure~\ref{fig: slalom curve} provides a clear visual comparison of this effect. There, we record the paths the humanoid traversed with a constant speed, as well as our speed controller output, and compare them with the desired reference path. The constant speed was selected so that the two runs have exactly the same completion time. Despite having the same average speeds, in the constant-speed run the humanoid has a hard time matching the speed during the steep turns and hits the wall at its corners. This does not happen with the adaptive speed run, which follows the desired path better.  


\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/planner/slalom_curve.pdf}
    \caption{\textbf{Comparison of planned paths} (blue) Our path with adaptive speed. (red) A path with a constant speed that has the same average speed as the adaptive-speed path. (dashed black) the desired reference path. %The constant speed was selected so that the two runs have exactly the same completion time. 
    When using a constant speed, the humanoid hits the wall at its corners. Using the adaptive speed generates a fast but smoother path, that is far from the obstacle but still follows follows well the desired path better.}
    \label{fig: slalom curve}
\end{figure}

For a quantitative evaluation of the Slalom test, we compare various constant speeds, as well as various configurations of our QP solver. The latter include different combinations of maximal lateral and longitudinal acceleration.  We summarize the results in Figures~\ref{fig: slalom pareto 1}-\ref{fig: slalom pareto 2}. Each choice of constant speed and QP configuration corresponds to a single point in the plots and is the average of 100 runs. The constant speeds were chosen between $1 \left[m/s\right]$ and $3.5 \left[ m/s\right].$ In Figure~\ref{fig: slalom pareto 1}, we report the success rate versus the average completion time. Success is defined as successfully reaching the target landmark. In Figure~\ref{fig: slalom pareto 2}, we show the same, but with the average 3D disposition error on the y-axis. As seen, our planner is Pareto-optimal in both measurements. That is, every QP configuration we tested enables the humanoid to traverse its path route faster at the same accuracy or at the same time, but with better accuracy, compared to an equivalent constant speed profile.
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.87\linewidth]{figures/planner/slalom_pareto1.pdf}
    \caption{\textbf{Failure rate and Completion Time: Pareto curve in the Slalom test}. Testing our speed controller vs. constant speed. Our planner obtains lower failure rate while retaining faster completion.}
    \label{fig: slalom pareto 1}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.87\linewidth]{figures/planner/slalom_pareto2.pdf}
    \caption{\textbf{Disposition error and Completion Time: Pareto curve in the Slalom test.} Testing our our speed controller vs. constant speed. Our planner obtains lower disposition error while retaining faster completion.}
    \label{fig: slalom pareto 2}
\end{figure}



\subsection{Randomized routes in a complex scene}\label{exp: full system}
Finally, we showcase \ourmethod{'s} ability to solve previously unseen scenes in varying forms. To do so, we constructed a scene consisting of: \textbf{(1)} multiple forms of terrains (smooth, gravel-like, and stairs), with \textbf{(2)} several types of obstacles (walls, low-ceiling, and a dynamic obstacle). Within this scene, we defined 4 landmarks. At each instantiation, \ourmethod{} is provided with a new and randomized route, consisting of a random ordering of landmarks and how they should be solved.

As shown in \cref{fig:teaser,fig: playground}, \ourmethod{} solves this task in varying forms while adhering to the scene constraints. It slows down and starts to crawl before passing under the low ceiling (top left), speeds up during straight lines while carefully slowing during a tight curve, and finally, it dynamically adapts the path when a collision with a dynamically moving object is deemed likely\footnote{The dynamic re-planning is best seen in the supplementary video.}.

% To showcase the full scope of our system, we devised a scene that requires the character to succeed in multiple aspects: 
% \begin{enumerate}
%     \item Navigating to various landmarks on the map forming a long scenario without failing.
%     \item Performing diverse types of motions along the route.
%     \item Completing the route quickly while handling sharp turns.
%     \item Avoiding static, top and dynamic obstacles.
% \end{enumerate}
% Our scene and a sample route and choice of motion types are given in Figure \ref{fig:teaser}. We include in the supplementary material multiple videos of the character following randomized routes and motion types in this scene, demonstrating the robustness and potential of our system. Screen captures are given in Figure \ref{fig: playground}.


% Now we add in the path planner. Explain the 3-4 domains we evaluate on.
% Quantitative experiments need to show success rates in solving the task (reaching the end).
% Qualitative experiments need to show (1) how the planner generates meaningful paths that aren't "trivial". (2) how it adapts the height to the 3D terrain. (3) how the character crawls under an obstacle. (4) the system adapts the entire motion to a dynamic obstacle (if we still intend to support this).


==> SIGGRAPH_2024/extra_figures.tex <==

\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/crawl_slope/frame10.jpg}}\hfill
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/crawl_slope/frame41.jpg}}\hfill
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/crawl_slope/frame49.jpg}}
         \caption{Crawling up a slope}
         \label{fig: locomotion crawl slope}
     \end{subfigure}\hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/crawl_gravel/frame65.jpg}}\hfill
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/crawl_gravel/frame76.jpg}}\hfill
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/crawl_gravel/frame89.jpg}}
         \caption{Crawling on gravel}
         \label{fig: locomotion crawl gravel}
     \end{subfigure}\hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/crawl_stairs/frame227.jpg}}\hfill
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/crawl_stairs/frame246.jpg}}\hfill
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/crawl_stairs/frame262.jpg}}
         \caption{Crawling down stairs}
         \label{fig: locomotion crawl stairs}
     \end{subfigure} \\
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/crouch_slope/frame117.jpg}}\hfill
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/crouch_slope/frame128.jpg}}\hfill
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/crouch_slope/frame136.jpg}}
         \caption{Crouch-walking up a slope}
         \label{fig: locomotion crouch slope}
     \end{subfigure}\hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/crouch_gravel/frame115.jpg}}\hfill
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/crouch_gravel/frame125.jpg}}\hfill
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/crouch_gravel/frame134.jpg}}
         \caption{Crouch-walking on rough terrain}
         \label{fig: locomotion crouch gravel}
     \end{subfigure}\hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/crouch_stairs/frame183.jpg}}\hfill
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/crouch_stairs/frame195.jpg}}\hfill
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/crouch_stairs/frame206.jpg}}
         \caption{Crouch-walking down stairs}
         \label{fig: locomotion crouch stairs}
     \end{subfigure} \\
          \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/walk_slope/frame80.jpg}}\hfill
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/walk_slope/frame89.jpg}}\hfill
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/walk_slope/frame97.jpg}}
         \caption{Walking up a slope}
         \label{fig: locomotion walk slope}
     \end{subfigure}\hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/walk_rough/frame53.jpg}}\hfill
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/walk_rough/frame63.jpg}}\hfill
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/walk_rough/frame77.jpg}}
         \caption{Walking on rough terrain}
         \label{fig: locomotion walk gravel}
     \end{subfigure}\hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/walk_stairs/frame318.jpg}}\hfill
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/walk_stairs/frame324.jpg}}\hfill
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/walk_stairs/frame336.jpg}}
         \caption{Walking down stairs}
         \label{fig: locomotion walk stairs}
     \end{subfigure} \\
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/run_slope/frame50.jpg}}\hfill
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/run_slope/frame56.jpg}}\hfill
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/run_slope/frame64.jpg}}
         \caption{Running up a slope}
         \label{fig: locomotion run slope}
     \end{subfigure}
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/run_gravel/frame71.jpg}}\hfill
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/run_gravel/frame76.jpg}}\hfill
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/run_gravel/frame82.jpg}}
         \caption{Running on rough terrain}
         \label{fig: locomotion run gravel}
     \end{subfigure}\hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/run_stairs/frame102.jpg}}\hfill
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/run_stairs/frame118.jpg}}\hfill
         \scalebox{-1}[1]{\includegraphics[width=0.33\textwidth]{figures/locomotion/run_stairs/frame123.jpg}}
         \caption{Running down stairs}
         \label{fig: locomotion run stairs}
     \end{subfigure}
     \caption{\textbf{Locomotion:} Screen captures of our trained controller when conditioned on various forms of locomotion across varying types of terrains. Crawling is achieved by requesting a head-height of $0.4 \left[m\right]$, crouching at $0.8 \left[m\right]$, walking and running at upright $1.47 \left[m\right]$. The corresponding speeds are $1 \left[m/s\right]$, $2 \left[m/s\right]$, $2 \left[m/s\right]$, and $4  \left[m/s\right]$.}
    \label{fig: locomotion example}
\end{figure*}

\begin{figure*}[h]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[trim={5cm 5cm 0cm 1cm},clip,width=\textwidth]{figures/full_system/slalom_wo.png}
         \caption{\textbf{Slalom test with constant speed (baseline).} The humanoid follows the path poorly, hitting the walls on every turn.}
         \label{fig: slalom naive}
     \end{subfigure}\hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[trim={5cm 5cm 0cm 1cm},clip,width=\textwidth]{figures/full_system/slalom_w.png}
         \caption{\textbf{Slalom test with adaptive speed (ours).} The humanoid follows the path well, never hitting the walls.}
         \label{fig: slalom dynamic}
     \end{subfigure}
     \caption{\textbf{Comparison of consistent and adaptive speed profiles on the slalom test.} The colors represent the speed, with red indicating speeds above 3.5m/s and blue below 1m/s.}
    \label{fig: slalom}
\end{figure*}

\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[trim={15cm 8cm 12cm 1cm},clip,width=\textwidth]{figures/full_system/random_2_waypoints.png}
         \caption{Starting at the tree: "Run to the car" then "walk to the swing" then "run to the bench" then "walk to the tree".}
         \label{fig: rand 2}
     \end{subfigure}\hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[trim={15cm 8cm 12cm 1cm},clip,width=\textwidth]{figures/full_system/random_8_waypoints.png}
         \caption{Starting at the car: "Walk crouching to the bench" then "walk crouching to the tree" then "walk crouching to the bench" then "walk crouching to the car".}
         \label{fig: rand 8}
     \end{subfigure}\\
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[trim={15cm 8cm 12cm 1cm},clip,width=\textwidth]{figures/full_system/random_15_waypoints.png}
         \caption{Starting at the car: "Crawl to the bench" then "crawl to the tree" then "walk crouching to the bench" then "sprint to the car"}
         \label{fig: rand 15}
     \end{subfigure} \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[trim={15cm 8cm 12cm 1cm},clip,width=\textwidth]{figures/full_system/random_21_waypoints.png}
         \caption{Starting at the car: "Run to the tree" then "walk to the swing" then "walk to the bench" then "run to the car".}
         \label{fig: rand 21}
     \end{subfigure}
     \caption{\textbf{Diverse solutions:} Our system can solve unseen tasks in diverse forms. Here, we show how the character traverses a random sequence of segments within the scene. Each example showcases a randomly sampled sequence of waypoints to be performed with a randomly sampled motion. The requested solution, for each segment, is described in the corresponding caption for each figure.}
    \label{fig: playground}
\end{figure*}


==> SIGGRAPH_2024/introduction.tex <==
\section{Introduction}

% For robots to realistically operate both in the real world and in virtual worlds, they need to understand the outcome of their actions. This demands physical simulation. However, physics is hard, prior work did very simple things. We take it a step further towards higher degrees of control and interactivity with the environment.

Animating human characters in complex environments is a challenging task, essential for various applications. These range from automating game design through simulating factories and urban areas to validating autonomous vehicles with pedestrian scenarios. Most existing studies on character animation apply kinematic models \cite{ling2020character, qing2023storytomotion}. Such models, while more forgiving, often struggle to accurately depict physical interactions with complex terrain, objects, or other characters.

In contrast, physics-based methods leverage simulation to ensure a physically realistic result. Previous research has largely focused on specific motion aspects, such as mimicking \cite{peng2018deepmimic}, interleaving motion types \cite{tessler2023calm}, and crowd simulation \cite{rempe2023trace}, rather than enabling characters to seamlessly navigate within comprehensive simulated worlds. 
%As a result, it is still unknown how to train physics-based models that can handle rich environments that contain 3D obstacles, complex terrain, and dynamic scenes.  

In this work, we address the problem of training physical motion models for humanoids in intricate settings. We devise an approach called \ourmethod{} for \textit{Plan and Move} that combines long-horizon path planning with a novel matching motion controller. This fusion creates an agent that responds to semantic instructions and is adept at navigating through various terrains and obstacles, including those that are static, dynamic, or impose height restrictions. It ensures that the humanoid navigates smoothly and human-like, avoiding obstacles along the path.

A key concept of our approach is that the long-term plan guides the motion controller through continuous physical properties, such as velocity and head height. The planner is aware of the performance envelope of the humanoid and plans a path through a series of planning layers.
\gald{the next description  mainly focuses on a* and makes the planning sound trivial. Instead we need to glorify our novel multi-stage planning, saying it hadn't been done before for physically-simulated humanoids.}
Initially, it employs an $A^*$ algorithm on a sparse grid \cite{Hart1968}, creating a basic path. This path is then refined to align with the humanoid's three-dimensional location and velocity at every moment. 
Finally, this path is fed into a trained motion controller that generates the intended actions. 
Refinement takes into account the performance envelope of the humanoid, generating a path that the motion controller can safely follow.

%These behaviors include running, walking, crouching, and crawling.
%Our methodology also extends to semantic analysis. After dividing the terrain into named segments (e.g., "Car" or "Bench"), the agent can follow instructions provided in templated language. \shie{say something about AV's and waypoint?}

% We propose a systematic approach to path and motion planning in rich simulated physical environments. 

% We consider the setup of a given environment that includes an uneven terrain, static, dynamic, and height-limiting obstacles. The terrain is partitioned to different named segments (like "Grass" or "Beach"). Our output is the actions of a humanoid agent affecting its joints. The agent's purpose is travelling to a desired segment in a human like motion, while avoiding the obstacles on its way.

% To solve this problem, 

The contributions of our work are as follows: (1) we introduce \ourmethod{}, a methodology for combining path planning and motion control within a detailed physical simulation. (2) Guided by structured semantic instructions, we present an efficient path-planning method. The planner takes into account scene information, producing a safe path across uneven terrain around static, dynamic, and three-dimensional obstacles. Additionally, (3), we develop a robust motion controller, trained through reinforcement learning. Training to imitate human motions, the controller produces motion tracking the requested path in a specified form.
\gald{based on our literature review, we can't see any prior art that employs long-term navigation and planning (with various motion types) of humanoids. We should clearly state we are the first.}

%\gald{For next time we write -- I don't think ended up stressing the novelties in the motion controller and how they uniquely match our planner. That is, unlike previous work, our motion controller (i) controls height and, as a consequence,  (ii) various motion types with the same policy.}


% The contributions of this paper are as follows:
% \begin{enumerate}
% \item A methodology for combining path planning and motion control within a detailed physical simulation, guided by structured semantic instructions.
% \item An efficient path-planner that effectively navigates around static, dynamic, and three-dimensional obstacles on uneven terrain. 
% \item The first text-conditioned diverse motions, like crouch-walking and crawling, on complex terrains with dynamic or 3D obstacles.
% %\item Our approach system operates on new scenes that were not observed during training.
% %trained motion controller generalizes to perform various locomotion types on unseen terrains. 
% \end{enumerate}


% \gald{
% \begin{enumerate}
% \item An efficient path-planning method that effectively navigates around static, dynamic, and three-dimensional obstacles on uneven terrain. 
% \item The first text-conditioned motion controller for diverse locomotion, like crouch-walking and crawling, on complex terrains.
% \item Our PlaMo agent is guided by structured semantic instructions. It navigates to chosen locations, bypasses static and dynamic obstacles, and maneuvers in requested forms.
% \end{enumerate}
% }









%In summary, our paper makes two main contributions. First, we developed a methodology for combining path planning and motion control  within detailed physical simulations, guided by structured semantic instructions. Specifically, we describe an efficient path-planning method that effectively navigates around static, dynamic, and three-dimensional obstacles on uneven terrain. It enables the motion controller, through adjustments in height and speed, to execute complex movements like crouch-walking and crawling, aligning with text instructions.

==> SIGGRAPH_2024/method.tex <==

\section{Method}\label{sec: method}
Our method, \ourmethod, consists of two main components (Figure \ref{fig:overview}):

\textbf{High-level path planner.} The planner receives two inputs: a physically simulated 3D scene and a templated text instruction describing a sequence of (locomotion type, start point, target point). The planner then outputs a path $\tau$ consisting of velocity and 3D head positions at each time-step. The path is optimized to lead the agent through a smooth path to reach the goal while avoiding obstacles. It is then sent to a motion controller.



%\gal{The following are not in figure 2, its explained in 4.2. I would remove this paragraph.} The planner consists of several sub-modules: (a) An A* algorithm on the granulated terrain, (b) a path refiner applying smoothing and obstacle avoidance, and (c) a speed controller for finding the optimal speed along the trajectory. 

\textbf{Low-level locomotion controller.} This controller receives as input the height map $h$ of the local terrain and a desired path $\tau$. It outputs a sequence of motor actions for the humanoid joints, resulting in the humanoid following the desired path. The locomotion controller is trained on real-world motion captures using RL to generate realistic human-like behavior. 

\textbf{Together}, at each time-step of the simulation, the %high-level dynamic 
path planner translates the current humanoid location and target landmark to a local path which the controller aims to follow. The controller then outputs actions on the joints to the simulator, which then advances to the next simulation step. %A diagram of our full system is given in Figure \ref{fig:overview}.


\begin{figure*}[ht]
\includegraphics[width=\textwidth]{figures/planner/planning.png}
  \caption{The three stages of our dynamic path planner: (i) $A^*$ solver, (ii) path refiner, and (iii) speed controller.}
  \label{fig:planning_diagram}
\end{figure*}

\subsection{Dynamic Path Planner}
\label{sec:planner}
We present a comprehensive module for path planning, structured into distinct phases. 
The full planning flow is visualized in Figure~\ref{fig:planning_diagram} (see also Figure \ref{fig:overview} for context). 

\textbf{Textual guidance parser.}
The input to the planner is a 3D simulated scene $\textit{Scene}$ and 
a series of $k$ text instructions in the form ``Run from the tree to the lake''. 
These instructions refer to known landmarks in the scene and we assign each landmark to the set of $(x,y)$ coordinates that correspond to it. 
%For example, a swing may cover a large area of the scene map than a bench . 
We then translate each instruction to a triplet of (source landmark, target landmark, locomotion type). Together, they form a sequence of instructions that go through the series of landmarks $L_1, \ldots,  L_k$. 

The output of our planner is a series of $k$ paths.
We observe that two main characteristics differentiate between desired forms of locomotion are speed and height. As such, each path is represented as a series of 3D positions. We determine velocities by controlling the distance between the points on the path. These paths are fed to the motion controller. 

The planner operates in three steps. 

\textbf{High-level planning with A*.} We first form a 2D-grid, connecting every point to its 8 neighbors. We then remove connections, such that where two adjacent locations are connected only if their height difference is below a limiting threshold, and none of the locations is part of a static obstacle. Then, for every landmark ${L_i}$, we mark all its assigned $(x,y)$ coordinates as goals for A*. 
Then, the A* algorithm \cite{bell2009hyperstar} constructs a shortest-path solution to the nearest coordinate of the landmark. %from every point on the grid \gal{Why do we need this? Sounds wasteful, we do have a single source location. Is it necessary to write this?} to the designated goal. Coupled with the agent's initial position $(x_0, y_0)$
%\gal{This should be the beginning point of the segment, not the beginning of the route (1st segemnt).}  
% we form a coarse, long-term, two-dimensional path to the goal. 
%To obtain smoother trajectories, we allow connectivity of every point in the grid with the $8$ points surrounding it which also includes diagonal transitions (with a corresponding distance cost). 
Due to its high computational cost, we perform the A* phase once and implement it using KD-trees. See more details about efficient reuse in the supplemental. 
%\gal{IF we do all to all points, we could do this once per scene?}, in the beginning of the run, and its output is used to any spawning position or perturbations in the agent's location. \gal{confusing . We did not discuss a case where there are mutuple spawns. I would simply remove this. }

\textbf{Path refiner.} The path created at the previous A* phase is rather coarse, and blind to dynamic and height obstacles. We refine it to achieve smoother paths that avoid all obstacles. 
For \textit{dynamic obstacles}, we detect potential collisions by estimating the movement pattern of the obstacle and comparing it with the last designated path $\tau$.
If a collision is likely to occur within a $1.5 \left[s\right]$ time frame, we replan the path, with the dynamic obstacle set in its future location as an added constraint. Finally, the path refiner adjusts the trajectory for smoothness and obstacle avoidance. 
It also adds to each frame the desired vertical (z-axis) head-height values that help the character navigate beneath height obstacles.

\textbf{Speed controller.} 
The path created at the previous two phases contains only spatial information and is blind to the performance envelope of the humanoid character. The third step aims to assign a velocity vector to each frame in the path, that is consistent both with the text guidance (different locomotion types have different speeds) and with the terrain (one should slow down during steep turns). Specifically, the third phase solves a quadratic programming problem (QP) designed to minimize travel time along the refined path. The QP is constrained by limits on valid speed range for each locomotion type, and by bounds on longitudinal and lateral accelerations that the humanoid character can achieve. This phase accounts for path curvature, and adapts longitudinal speed based on the lateral acceleration. The result is that the agent slows down before turns. Furthermore, the speed controller adjusts the speed according to the elevation at each path point, resulting in a speed profile for each waypoint on the refined 3D path.



\subsection{Locomotion controller}
\label{sec:controller}

\begin{figure}[hb]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/ww_controller}
    \caption{\textbf{Locomotion module.} The locomotion policy observes the character state $s_t$, the height map of the terrain $h$, and the requested path $\tau$. During training, the trajectories are randomly sampled, whereas in inference they take into account the terrain characteristics, such as obstacles. The resulting state, after simulating the predicted action, is used both for providing the style reward $r^\text{amp}$ and the path following reward $r^\tau$.}% \gal{It would be useful ot make this figure larger. Perhaps make it shorter in height so we can put it full page? or the opposite, make it more narrow, so it takes more text lines? }}
    \label{fig: locomotion}
\end{figure}

%We complement the path planner with a low-level physics-based controller to successfully generate full-body physical animation. 
The locomotion controller is constructed to generate human-like physical motion. It needs to do so while adhering to the requested motion traits, and traversing diverse non-trivial terrains. For that purpose, we train an RL agent. Our reward function is composed of two components -- one for following the path and the second for producing realistic motion. In this paper, we accommodate four forms of locomotion: running, walking, crouch-walking, and crawling. A diagram of the locomotion module is given in Figure~\ref{fig: locomotion}.

\textbf{Robust control through RL.} Similar to previous work \cite{rempe2023trace,hassan2023synthesizing}, we model the problem through goal-conditioned RL. Here, the goal-conditioned policy is trained to track a target path $\tau$, generated by the planner as explained in Section~\ref{sec:planner} above. We observe that two main characteristics differentiate between our desired forms of locomotion -- speed and height. As such, the path is constructed in 3D, where at each time step $t$ the point $\tau_t$ represents the 3D coordinates for the head. By controlling the distance between the points, we can determine the requested speed, and changing the $Z$-axis provides easy control for the requested character height. 

Due to the importance of height control, we split the reward into two components. The first considers the $x$-$y$ displacement of the character. This guides the path the character should follow, in addition to speed. The second component considers the height of the head.
\begin{equation*}
    r_t^\tau = 0.5 e^{- c_\text{pos} || \tau_t^{x,y} - s_t^{x,y} ||^2} + 0.5 e^{- c_\text{height} || \tau_t^z - s_t^z ||^2} \, ,
\end{equation*}
where $c_\text{pos}=2$ and $c_\text{height}=10$ are fixed weight coefficients.

To successfully move across diverse terrains, the controller needs to be aware of changes in the terrain around it. Similarly to \citet{rempe2023trace}, we provide it with a height grid $h_t$ representing the height of the terrain around the character, relative to its global position. This grid represents 64 samples (8 by 8) spanning $0.8 \left[m\right]$ on each horizontal axis.

\textbf{Adversarial learning.} While the target trajectory provides an intuitive control mechanism for the agent, by itself it does not ensure the realism of the resulting motions. Complementing the task reward, we use the same design as in AMP \cite{peng2021amp}. AMP uses a discriminator, which is trained to differentiate between ground-truth motions and simulated motions generated by our agent. The resulting reward combines the reward obtained by tracking the objective, with the discriminative reward:
\begin{equation*}
    r_t = r_t^\text{amp} + r_t^\tau \,.
\end{equation*}

\textbf{Motion curation.} The adversarial reward in AMP is maximized when the pose distribution induced by the control policy matches that of the data. Naively providing a diverse dataset of human motions may result in unwanted behaviors, since, for example, performing back-flips and break-dancing is not required for locomotion. To ensure that the motion distribution matches the expected motions needed to solve the task, we hand-picked 75 distinct motions from the AMASS dataset \cite{AMASS:ICCV:2019}, covering the 4 forms of locomotion, performed in various styles. An ablation study of this choice is presented in Section \ref{sec: experiments}.

% The correlation between data and task works both ways. 
\textbf{Motion-aware path generation.} During training, the path generator samples random paths for the character to follow as a task. If the task demands unlikely motion characteristics given the data, the motion becomes unrealistic and results in overall performance degradation. For example, assume that the task is crawling at $v=5 m/s$ (fast running speed). This kind of movement is unrealistic and, therefore, will not show in our motion capture data. Thus, the task reward and discriminative reward will contradict each other, impairing the training process.

To encourage the correlation of reward components, we ensure a tight coupling between the requested height and speed. First, the path generator samples the requested height for each point along the path. The height is sampled such that it is random between $0.4$ (crouching) and $1.47$ (standing upright), with smooth transitions in-between. Then, the speed is sampled uniformly between $0$ and $v_t^{\max{}}$, where:
\begin{equation*}
    v_t^\text{max} = \min{(1 + 4 \cdot (z_t - z^\text{min}) / (1.2 - z^\text{min}),\, V_{\max{}})} \,,
\end{equation*}
for a minimal height $z^\text{min} = 0.4\left[m\right]$ and maximal speed $V_{\max{}}=5 \left[m/s\right]$. That is, the maximum speed increases linearly from $v_t^\text{max}=1 \left[m/s\right]$ when the requested height is $0.4 \left[m\right]$, up to $v_t^\text{max}=5\left[m/s\right]$ for any height above $1.2\left[m\right]$ (humanoid height is $1.47 \left[m\right]$).



==> SIGGRAPH_2024/related-work.tex <==
\section{Related Work}

\textbf{Physics-based animation.} As evident by prior works, physics-based controllers learn robust reactive policies \cite{zhang2023learning,yuan2019ego,yuan2020residual,luo2022embodied,luo2023perpetual}. These policies adapt to changes in the scene such as irregular terrain, obstacles, and adversarial perturbations \cite{wang2020unicon,lee2023questenvsim,luo2023universal}. Typically, physics-based controllers focus on complex motions in simple scenes \cite{peng2022ase, tessler2023calm, juravsky2022padl}, or simple motions within complex scenes \cite{rempe2023trace, hassan2023synthesizing}. Perhaps closest to our work is TRACE and PACE \cite{rempe2023trace}, which focuses on pedestrian locomotion with a diffusion-based planner. To generate paths, TRACE (the planning module in \citet{rempe2023trace}) is trained on pedestrian data, typically walking motions in scenes without height-based obstacles. In contrast, here we focus on long-term 3D-aware navigation and locomotion. \ourmethod{} combines a short-sighted terrain-aware locomotion controller with a long-term and adaptive scene-aware path generator. The path generator plans a 3D trajectory for the humanoid, controlling both speed and height. It does so while avoiding obstacles, both static and dynamic while adhering to external motion constraints. Provided the path, our motion controller generates motor actuations to track the requested path along rich and complex terrains.

% \assaf{Why not trace from PACER? TRACE requires real world data of pedestrians for behavior control. In our case the obstacles have a simple motion, and the motion can be constrained (crawling, crouching), for which data does not exist.}

\textbf{Scene aware animation.} Prior work has used kinematic-animated characters to tackle a wide range of problems such as object interaction \cite{starke2019neural, li2023object}, long-term motion generation \cite{ling2020character} and storytelling \cite{qing2023storytomotion}. However, as physics-based animation is less forgiving, these works have typically focused on solving specific object-interaction tasks \cite{hassan2023synthesizing}, or simple locomotion (walking or running) with short-term planning across complex terrains \cite{rempe2023trace}. We tackle the problem of long-term motion generation across complex scenes using physics-based control.

\textbf{Motion planning. } There are numerous works in the world of planning motion in different levels of hierarchy. For high-level planning, the A* algorithm and its variations \cite{bell2009hyperstar, yao2010path, duchovn2014path} use dynamic programming to produce a discrete path that considers the cost and connectivity of moving across the grid. Finer control models such as Model Predictive Control (MPC; \cite{qin1997overview, holkar2010overview}) construct an optimization problem by considering the dynamics of all objects and the physical constraints of the agent while using a lookahead of a receding horizon, these models usually require an explicit knowledge on the dynamics of the agent itself. In cases where the dynamics of the agent or objects in the scene are unknown or complicated, learning methods can be employed instead such as RL for a given simulator \cite{michels2005high, chen2022deep} or diffusion models when there is access to relevant data \cite{barquero2023belfusion, karunratanakul2023guided}. Our works are most related to recent approaches for planning in autonomous driving, which extend A* with additional smoothing and obstacle avoidance modules to form feasible trajectories \cite{yeong2020development, zhong2020hybrid, maw2020iada}. 

%\chen{Goal here is to motivate physics based animation. We want to say (1) prior work showed that physics based animation can learn robust reactive policies. These policies adapt to changes in the scene (object, terrain, adversarial perturbations). However, these works typically focus on complex motions in simple scenes -- ASE, CALM, PADL, PHC; or simple motions within complex scenes -- PACER, InterPhys.}\chen{Also need to talk about how these methods solve very specific tasks.}\chen{In this work we tackle long-term planning with improved motion control across complex scenes.}\chen{should probably mention that PACER takes a step in this direction, but only considers locomotion as they focus on pedestrians, however in many problems both indoors and outdoors, especially in games, it is of great interest to have 3D awareness and motion.}


%\textbf{Scene aware animation.} \chen{Here we have two lines of work. (1) kinematic models. they have tackled a very wide range of problems. GalC shared some in the WW channel, interacting with objects, long-term motion generation Scene something, etc... (2) physics based, where it is much more challenging as the problem is control. The results are much higher quality and generalize better but harder to achieve. In this work we tackle long-term motion generation across complex scenes using physics-based.}



==> overview_bak.tex <==

\input{training_fig}

\section{Overview}\label{sec: overview}

% Overview of the system. We have 3 components -- semantic parser, dynamic path planner, and locomotion controller.
% Brief explanation how each is used and how it is obtained.
Here we provide an overview of the entire system, where in the next section we will delve into more details. Our system is composed of two main components.

\textbf{Low-level locomotion controller. }The low-level controller receives as input the local terrain's height map $\mathcal{M}$ and a desired path $\tau$. The output is the actions on the humanoid joints resulting in the humanoid following the desired path. The locomotion is trained on real world motion captures using RL to generate realistic human-like behavior. 

\textbf{High-level dynamic path planner.} Given a desired goal location, the dynamic path planner outputs a path $P$ to the low-level controller each time step to form continuous control. The path should lead the agent through a smooth trajectory to reach the goal while avoiding obstacles. The planner is composed of several sub-modules: (a) An A* algorithm on the granulated terrain, (b) a path refiner applying smoothing and obstacle avoidance, and (c) a quadratic programming (QP) solver for finding the optimal speed along the trajectory. 

In each time-step of the simulation, the high-level dynamic path planner translates the current goal segment to a local path which the controller aims to follow. The controller then outputs actions on the joints to the simulator which then advances to the next simulation step. diagram of our system is given in Figure \ref{}.





==> training_fig.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/pipline}
    \caption{\textbf{Method overview.}}
    \label{fig:overview}
\end{figure*}
